Vulnerable Open Source Dependencies: Counting Those That Matter

BACKGROUND: Vulnerable dependencies are a known problem in today's open-source software ecosystems because OSS libraries are highly interconnected and developers do not always update their dependencies. AIMS: In this paper we aim to present a precise methodology, that combines the code-based analysis of patches with information on build, test, update dates, and group extracted from the very code repository, and therefore, caters to the needs of industrial practice for correct allocation of development and audit resources. METHOD: To understand the industrial impact of the proposed methodology, we considered the 200 most popular OSS Java libraries used by SAP in its own software. Our analysis included 10905 distinct GAVs (group, artifact, version) when considering all the library versions. RESULTS: We found that about 20% of the dependencies affected by a known vulnerability are not deployed, and therefore, they do not represent a danger to the analyzed library because they cannot be exploited in practice. Developers of the analyzed libraries are able to fix (and actually responsible for) 82% of the deployed vulnerable dependencies. The vast majority (81%) of vulnerable dependencies may be fixed by simply updating to a new version, while 1% of the vulnerable dependencies in our sample are halted, and therefore, potentially require a costly mitigation strategy. CONCLUSIONS: Our case study shows that the correct counting allows software development companies to receive actionable information about their library dependencies, and therefore, correctly allocate costly development and audit resources, which is spent inefficiently in case of distorted measurements.

==> impact.tex <==
In an industrial setting, the practical negative impact of using an \emph{inadequate} measurement method can be substantial. Ensuring a healthy supply chain of third-party dependencies (of which the large majority is FOSS)
is a continuing effort that spans the development and the operational phases of a product lifetime.

As part of SAP's secure development life-cycle, all development projects go through several validation steps and
each single finding has to be audited, assessed, and mitigated.
After the product is released to customers, and for its entire
operational lifetime, its own security and the security of its third-party dependencies are continuously monitored. When a vulnerability is detected in one of the dependencies, timely mitigations need to be developed and deployed to all affected systems. In the case of FOSS dependencies,
these mitigations may consist of dependency updates, or in ad-hoc fixes in the product that relies on the affected
library or in the dependency itself (through a company-internal fork, that can be temporary or persistent). When the product portfolio of a company includes thousands of products, whose support period can extend to decades,
wrong assessments lead to inadequate risk management and inefficient allocation of resources, which ultimately translate to increased chances of security incidents and financial loss.

The distinction between deployed and non-deployed components allows quick and reliable pre-filtering of not exploitable vulnerable dependencies, since they are not part of the deployed product.
From our analysis of a sample of over 550 SAP development projects, as many as 20\% of all the dependencies are \emph{non-deployed}.

The granularity at which dependencies are analyzed and the reliability with which vulnerabilities affecting them are detected are essential to obtaining a meaningful
view of the (security) health of the dependencies of a project. 
Approaches that use imprecise vulnerability detection methods and that ignore the interdependencies among the individual nodes of the dependency tree yield a distorted view, which requires
tedious, manual reviews to be correctly interpreted and that cause precious resources to be wasted. Failing to group dependency nodes that belong to the same group (e.g., to the same FOSS project), and that are updated together, makes the update of certain libraries appear more problematic than it is. The vulnerability may affect a node that is deep in the dependency tree, while the node that the application developer would need to update might be much shallower (e.g., it could even be a direct dependency). More in general, imprecise approaches to vulnerability management undermine the trust of developers on automated  analysis because the dependencies identified as problematic do not correspond to those that must be actually acted upon to address the reported issues. As a consequence, despite the promises of automation, considerable additional human effort and expert judgment is required to determine the appropriate mitigation strategy.

Finally, determining precisely whether a dependency could be upgraded to a non-vulnerable version or not (because such a version does not exist, and perhaps will never exist, if the dependency is no longer maintained) is the key to choosing the correct mitigation strategy.
Addressing vulnerabilities in FOSS components that are alive, but for which a fixed release does not exist \emph{yet}, requires to act fast, so that an emergency solution
can be rolled-out as fast as possible to all customers. Being temporary and urgent, such mitigation might not be optimal. An upgrade to a non-vulnerable version of the dependency will eventually be done.
Conversely, if a vulnerability affects a dependency that is no longer maintained, fixing the code of the dependency would effectively mean creating a company-internal fork, whose long-term support could require substantial additional investments and maintenance effort.


==> replicability.tex <==
We highly encourage to reproduce the results of this study and to ease this task we are going to release the tool we developed  to resolve and compute software dependencies under an open-source license. The vulnerability database used in this paper is property of SAP. However, the interested reader can follow the instructions on how such a database could be reconstructed (Section~\ref{sec:vuln:identification}). Moreover, the information about vulnerabilities may be obtained from sources such as the NVD and from commercial tool vendors, such as Snyk and Sourceclear, who grant a free access to parts of their vulnerability databases.
\as{well, there is another piece that is missing to replicate the study: Vulas; and the same cannot be
achieved with another tool (not with the same precision, at least)}
